Forward Invariance of Sets for Hybrid Dynamical Systems (Part I)

In this paper, tools to study forward invariance properties with robustness to dis- turbances, referred to as robust forward invariance, are proposed for hybrid dynamical systems modeled as hybrid inclusions. Hybrid inclusions are given in terms of dif- ferential and difference inclusions with state and disturbance constraints, for whose definition only four objects are required. The proposed robust forward invariance notions allow for the diverse type of solutions to such systems (with and without dis- turbances), including solutions that have persistent flows and jumps, that are Zeno, and that stop to exist after finite amount of (hybrid) time. Sufficient conditions for sets to enjoy such properties are presented. These conditions are given in terms of the objects defining the hybrid inclusions and the set to be rendered robust forward invariant. In addition, as special cases, these conditions are exploited to state results on nominal forward invariance for hybrid systems without disturbances. Furthermore, results that provide conditions to render the sublevel sets of Lyapunov-like functions forward invariant are established. Analysis of a controlled inverter system is presented as an application of our results. Academic examples are given throughout the paper to illustrate the main ideas.

==> Sections/SuffConds-AL.tex <==
Definition~\ref{def:rwFI} and Definition~\ref{def:rFI} state that a set enjoys robust forward invariance properties when the state evolution stays within the set regardless of the value of the disturbance.
When disturbance signals are $w_c \equiv 0$ and $w_d \equiv 0$, Definition~\ref{def:FI} reduces to nominal forward invariance properties for $\HS$ given as in \eqref{eq:H}.
Verifying these properties for a given set using the definitions requires to solve for solution pairs to $\Hw$, and solutions to $\HS$, respectively, explicitly.
To circumvent that challenge, we present, when possible, solution-independent conditions to guarantee each notion.

For clarity of exposition, in Section~\ref{sec:HSuffConds}, we provide sufficient conditions for the nominal cases, which are firstly proposed in \cite{120}.
Then, in Section~\ref{sec:HwSuffConds}, these conditions are extended to hybrid systems with generic disturbance signals, i.e., $\Hw$ given as in \eqref{eq:Hw}.

\vspace{-4mm}

\subsection{Sufficient Conditions for Nominal Forward Invariance Properties for $\HS$}
\label{sec:HSuffConds}
We present the sufficient conditions for forward invariance of a given set $K$ for $\HS$ that involve the data $\data$.
For the discrete dynamics, namely, the jumps, such conditions involve the understanding of where $G$ maps the state to.
Inspired by the well-known Nagumo Theorem \cite{nagumo1942lage}, for the continuous dynamics, namely, the flows, our conditions use the concept of tangent cone to the closed set $K$.
The tangent cone at a point $x \in \reals^n$ of a closed set $K \subset \reals^n$ is defined using the Dini derivative of the distance to the set, and is given by\footnote{In other words, $\omega$ belongs to $T_K(x)$ if and only if there exist sequences $\tau_i \searrow 0$ and $\omega_i \rightarrow \omega$ such that $x + \tau_i \omega_i \in K$ for all $i \in \nats$; see also \cite[Definition 1.1.3]{aubin.viability}. The latter property is further equivalent to the existence of sequences $x_i \in K$ and $\tau_i > 0$ with $x_i \rightarrow x, \tau_i \searrow 0$ such that $\omega = \lim_{i\to\infty} (x_i - x)/\tau_i$.}
\ConfSp{-5mm}
	\begin{align}\label{eq:tangent}
		T_K(x) = \left\{ \omega \in \reals^n : \liminf\limits_{\tau \searrow 0} \frac{|x+\tau \omega|_K}{\tau} = 0 \right\}.
	\end{align}
In the literature (see, e.g., \cite[Definition 4.6]{jahn1994tangent} and \cite{aubin.hs.viability}), this tangent cone is also known as the sequential Bouligand tangent cone or contingent cone.
In contrast to the Clarke tangent cone introduced in \cite[Remark 4.7]{jahn1994tangent}, which is always a closed convex cone for every $x \in K$, the tangent cone (possibly nonconvex) we consider in this work includes all vectors that point inward to the set $K$ or that are tangent to the boundary of $K$.\footnote{Note that, for a convex set, the Bouligand tangent cone coincides with the Clarke tangent cone.}

Our sufficient conditions for forward invariance require part of the data of $\HS$ and the set $K$ to satisfy the following mild assumption.
%In particular, the following properties are also key in guaranteeing existence of solutions.
\begin{assumption}\label{assum:data}
	The sets $K, C$, and $D$ are such that $K \subset \overline{C}\cup D$ and that $K \cap C$ is closed \chai{$C$ is closed}.
	The map $F: \reals^n \rightrightarrows \reals^n$ is outer semicontinuous, locally bounded relative to $K \cap C$, and $F(x)$ is nonempty and convex for every $x \in K \cap C$.
\end{assumption}
\chai{
	In addition, for ease of representation, we denote the set that collects all points in the flow set that \ref{item:VC} does not hold as
	$L : = \{x \in C: F(x) \cap T_C(x)\}$.
}

The following result is a consequence of the forthcoming Theorem~\ref{thm:rwFI} in Section~\ref{sec:HwSuffConds} and its proof will be delayed to that section.

Sufficient conditions for a given set $K$ to be weakly forward pre-invariant and weakly forward invariant are presented.
\begin{theorem}(nominal weak forward pre-invariance and weak forward invariance)\label{thm:wfi}
	Given $\HS= \data$ as in \eqref{eq:H} and a set $K$, suppose $K, C, D,$ and $F$  satisfy Assumption~\ref{assum:data}.
	The set $K$ is weakly forward pre-invariant for $\HS$ if the following conditions hold:
	\begin{enumerate}[label = \ref{thm:wfi}.\arabic*), leftmargin=2.8\parindent]
		\item\label{item:wfi1} For every $x \in K \cap D$, $G(x) \cap K \neq \emptyset$;
		\item\label{item:wfi2} For every $\chai{x \in \hC : = K \setminus (L\cup D)}$, $F(x) \cap T_{K \cap C}(x) \neq \emptyset$.
	\end{enumerate}
	Moreover, $K$ is weakly forward invariant for $\HS$ if, in addition\chai{, the following holds:}
	\begin{enumerate}[label = N$\star$\arabic*), leftmargin=2\parindent]
		\item\label{item:NL} $K \cap L \subset D$.
		\item\label{item:N*} For every \chai{$\phi \in \sol_{\HS}(\hC)$} with $\rge \phi \subset K$, case \ref{item:b.2n} in Proposition~\ref{prop:existence} does not hold.
	\end{enumerate}
\end{theorem}

\vspace{-1mm}
The next result, which is a consequence of Theorem~\ref{thm:rFI} in Section~\ref{sec:HwSuffConds} provides sufficient conditions for a set $K$ to be forward pre-invariant and forward invariant for $\HS$.
\begin{theorem}(nominal forward pre-invariance and forward invariance)\label{thm:fi}
	Given $\HS= \data$ as in \eqref{eq:H} and a set $K \subset \reals^n$. Suppose $K, C, D,$ and $F$ satisfy Assumption~\ref{assum:data} and that 
	$F$ is locally Lipschitz on $C$.
	The set $K$ is forward pre-invariant for $\HS$ if the following conditions hold:
	\begin{enumerate}[label = \ref{thm:fi}.\arabic*), leftmargin=2.8\parindent]
		\item\label{item:fi1} $G(K \cap D) \subset K$;
		\item\label{item:fi2} For every \chai{$x \in \hC : = (K \cap C)\setminus L$}, $F(x) \subset T_{K \cap C}(x)$.
	\end{enumerate}
	Moreover, $K$ is forward invariant for $\HS$ if, in addition, \chai{\ref{item:NL} and \ref{item:N*} in Theorem~\ref{thm:wfi} hold.}
\end{theorem}

The following example is used to illustrate Theorem~\ref{thm:wfi} and Theorem~\ref{thm:fi}.
\begin{example}[solutions with finite escape time]\label{ex:pre}
	Consider the hybrid system $\HS = \data$ in $\reals^2$ with system data given by
	\IfConf{
	$F(x) :=(1 + x_1^2, 0)$ for every $x \in C:= \{ x \in \reals^2: x_1 \in [0, \infty), x_2 \in [-1,1] \}$ and $G(x) := (x_1+ \ball, x_2)$ for every $x \in D:= \{ x \in \reals^2: x_1 \in [0, \infty), x_2 = 0 \}.$
	}{
	\begin{align*}
	& F(x) := \begin{bmatrix} 1 + x_1^2\\ 0 \end{bmatrix} 
	& \forall x\in C := \{ x \in \reals^2: x_1 \in [0, \infty), x_2 \in [-1,1] \},\\
	& G(x) := \begin{bmatrix} x_1+ \ball \\ x_2 \end{bmatrix}
	& \forall x\in D := \{ x \in \reals^2: x_1 \in [0, \infty), x_2 = 0 \}.
	\end{align*}
}
Let $K = C$ and note the following properties of maximal solutions to $\HS$:
\begin{itemize}[leftmargin = 4mm]
	\item For some $x \in K$, there exists $\phi = (\phi_1, \phi_2) \in \sol_\HS(x)$ with $\rge \phi \subset K$, but is not complete due to $\lim\limits_{t \searrow t^*}\phi_1(t,0) = \infty$ with $t^* <\infty$; for instance, from $x = (0, 1)$, the solution given by $\phi(t,0) = (\tan(t), 1)$ for every $(t,0) \in \dom \phi$ has its $\phi_1$ component escape to infinite as $t$ approaches $t^* = \pi/2$;\footnote{Note condition \ref{item:N*} does not hold for $\HS$ in Example~\ref{ex:pre}, and the solutions that have a finite escape time are maximal but not complete as described in case \ref{item:b.2n} in Proposition~\ref{prop:existence}.}
	\item From points in $D \subset K$, there exist maximal solutions that leave $K$ and are not complete: such maximal solutions end after a jump because their $x_1$ component is mapped outside of $K$.
\end{itemize}
Thus, we verify weak forward pre-invariance of $K$ by applying Theorem~\ref{thm:wfi}.
\vspace{-3mm}
	\begin{figure}[h]
		\centering
%		\setlength{\unitlength}{.3\textwidth}
		\includegraphics[width=\figsize]{pre_FI.eps}
		\small
		\put(-0.03,.33){$x_1$}
		\put(-1.01,.65){$x_2$}
		\put(-.98,.53){1}
		\put(-.98,.05){-1}
		\put(-.98,.26){0}
		\put(-.7,.17){$C$}
		\put(-.36,.35){$D$}
		\put(-1,.35){$x_v$}
		\put(-.83,.32){$T_{K\cap C}(x_v)$}
		\put(-.62,.58){$x_u$}
		\put(-.5,.5){$T_{K\cap C}(x_u)$}
		\put(-.47,.03){$x_l$}
		\put(-.35,.1){$T_{K\cap C}(x_l)$}
		\caption{Flow and jump sets of the system in Example~\ref{ex:pre}.}
		\label{fig:propwppfi}
	\end{figure}
\vspace{-2mm}

\noindent The sets $K, C, D$ and the map $F$ satisfy Assumption~\ref{assum:data} by construction and condition \ref{item:wfi1} holds for $\HS$ by definition of $G, D$ and $K$.
Condition \ref{item:wfi2} holds because for every $x \in K \cap C$,  $F(x)$ points horizontally, and
\IfConf{
	$$T_{K \cap C} (x) = \begin{cases}
	\reals \times \reals_{\leq 0} & \ifeq x_1 \in (0, \infty), x_2 = 1\\
	\reals \times \reals & \ifeq x_1 \in (0, \infty), x_2 \in (-1,1)\\
	\reals \times \reals_{\geq 0} & \ifeq  x_1 \in (0, \infty), x_2 = -1\\
	\reals_{\geq 0} \times \reals_{\leq 0} &\ifeq x = (0,1)\\
	\reals_{\geq 0} \times \reals &\ifeq x_1 = 0,  x_2 \in (-1,1)\\
	\reals_{\geq 0} \times \reals_{\geq 0} & \ifeq x =(0,-1).
	\end{cases}$$
}{
$$T_{K \cap C} (x) = \begin{cases}
\reals \times \reals_{\leq 0} & \ifeq x \in  \{ x \in \reals^2: x_1 \in (0, \infty), x_2 = 1\}\\
\reals \times \reals & \ifeq x \in  \{ x \in \reals^2 : x_1 \in (0, \infty), x_2 \in (-1,1)\}\\
\reals \times \reals_{\geq 0} & \ifeq x \in  \{ x \in \reals^2: x_1 \in (0, \infty), x_2 = -1\}\\
\reals_{\geq 0} \times \reals_{\leq 0} &\ifeq x = (0,1)\\
\reals_{\geq 0} \times \reals &\ifeq x \in  \{ x \in \reals^2: x_1 = 0,  x_2 \in (-1,1)\}\\
\reals_{\geq 0} \times \reals_{\geq 0} & \ifeq x =(0,-1).
\end{cases}$$
}
Tangent cones of $K \cap C$ at the boundary points $x_u, x_v$ and $x_l$ of $K$ are shown in Figure~\ref{fig:propwppfi}.

Now, consider the same data but with $G$ replaced by $G'(x) = G(x) \cap (\reals_{\geq 0} \times \reals)$ for each $x \in D$.
The set $K = C$ is forward pre-invariant for this system.
This is because maximal solutions are not able to jump out of $K$ as $G'$ only maps $x_1$ components of solutions to $[0, +\infty)$.
More precisely, the conditions in Theorem~\ref{thm:fi} hold: we have $G'(D \cap K) \subset K$, and Assumption~\ref{assum:data} and condition \ref{item:fi2} hold as discussed above.
\hfill $\triangle$
\end{example}

\begin{remark}
	The hybrid inclusions framework allows for an overlap between the flow set $C$ and the jump set $D$.
	As a result, the proposed conditions are not necessary to induce forward invariance properties of sets for $\HS$.
	When existence of nontrivial solutions and completeness are not required for every point in $K$, as in the ``pre'' notions, some of these conditions are necessary.
	In fact, suppose $K,C,D$, and $F$ satisfy Assumption~\ref{assum:data}:
	\begin{itemize}[leftmargin = 4mm]
		\item If $K$ is weakly forward pre-invariant for $\HS$, then for every
%\ricardo{My initial take on this was that it should be $\overline{C}$ instead of $C$ in this condition, so that flows into $K \cap C$ are not possible. But the trick seems to be that flows into $K \cap C$ cannot happen from points $x \in (K \cap D)\setminus C$ that are also in $\partial C$ since those would not be in $K \cap C$, which seems is closed, flow into it would not be possible:}
		$x \in (K \cap D)\setminus C$, we have $G(x) \cap K \neq \emptyset.$
		\item If $K$ is forward pre-invariant or forward invariant for $\HS$, then condition \ref{item:fi1} in Theorem~\ref{thm:fi} holds.
		\item If $K$ is weakly forward invariant or forward invariant for $\HS$, then condition \ref{item:wfi2} in Theorem~\ref{thm:wfi} holds.\footnote{A similar claim is presented in \cite[Proposition 3.4.1]{aubin.viability} for continuous-time system.}
	\end{itemize}
	%For the ``non-pre'' notions, since \ref{item:wfi2} guarantees (VC) on $K \setminus D$ and \ref{item:VC} in Proposition~\ref{prop:existence} is necessary to guarantee the existence of nontrivial solutions from every point in $K$.
	Moreover, unlike \cite[Theorem 3]{aubin.hs.viability}, when the flow map $F$ is Marchaud\footnote{A map $F$ is Marchaud on $K \cap C$ when Assumption~\ref{assum:data} holds and $F$ has linear growth; see \cite[Definition 2.2.4]{aubin.viability}.} and Lipschitz as defined in Definition~\ref{def:lip}, condition \ref{item:fi2} in Theorem~\ref{thm:fi} is not necessary
	as the following example shows.
%	\begin{example}\label{ex:counterTangent}
		Consider $\HS = \data$ in \eqref{eq:H} with data 
		$F(x) =
		\begin{cases}
		1 & \ifeq x > -1\\
		[-1,1] & \ifeq x = -1
		\end{cases}$ 
		for each $x \in C : = [-1, 1]$, $G(x) := \{-1, 0\}$ for each $x \in D: = \{1\}$.
		By inspection, the set $K = C$ is forward invariant for $\HS$ and $F$ is Marchaud and Lipschitz.
		However, condition \ref{item:fi2} in Theorem~\ref{thm:fi} does not hold for every $x \in K \cap C$ -- it does not even hold on 
		$(K \cap C)\setminus D$, which are the points where flows are possible.
%	\end{example}
\end{remark}

\vspace{-4mm}

\subsection{Sufficient Conditions for N$\star$)}\label{sec:nstar}
In Theorem~\ref{thm:wfi} and Theorem~\ref{thm:fi}, item \ref{item:N*} excludes case \ref{item:b.2} in Proposition~\ref{prop:wexistence}, where solutions escape to infinity in finite time during flows.
Hence, when every solution $\psi$ to $\dot{x} \in F(x)$ with $x \in K \cap C$ does not have a finite escape time, namely, there does not exist $t^* < \infty$ such that $\lim\limits_{t \searrow t^*} |\psi(t)| = \infty$, then item \ref{item:N*} holds for $K$ and $\HS$.
Although, in principle, item \ref{item:N*} is a solution-dependent property, it can be guaranteed without solving for solutions when $F$ is single valued and globally Lipschitz.
Moreover, we provide several other alternatives in the next result.
\begin{lemma}(sufficient conditions for completeness)\label{lem:star}
	Given $\HS = \data$ and a set $K\subset \reals^n$, suppose $K, C, D,$ and $F$ satisfy Assumption~\ref{assum:data} and item \ref{item:wfi2} in Theorem~\ref{thm:wfi}.
	Condition \ref{item:N*} in Theorem~\ref{thm:wfi} holds if
	\begin{enumerate}[label = \ref{lem:star}.\arabic*), leftmargin=2.8\parindent]
		\item\label{item:star1} \chai{$\hC$} is compact; or
		\item\label{item:star2} $F$ is bounded on \chai{$\hC$}; or
		\item\label{item:star3} $F$ has linear growth.
	\end{enumerate}
\end{lemma}
\chai{Item \ref{item:star2} and \ref{item:star3} redundant? The following proof needs to be updated:
\begin{proof}
	Let $\phi \in \sol_{\HS}(K \cap C)$ with $\rge \phi \subset K$ be as described by \ref{item:b.2} in Proposition~\ref{prop:existence}; namely, $t \mapsto \phi(t,J)$ defined on $I^J$, where $(T,J) = \sup \dom \phi, T+ J < \infty$ and, for some $t^J, I^J = [t_J, T)$.
	Since $t \mapsto \phi(t,J)$ is locally absolutely continuous on $I^J$, $\lim\limits_{t \rightarrow T} \phi(t,J)$ is finite or infinity.
	If it is finite, then $t \mapsto \phi(t,j)$ can be extended to $\overline{I^J}$, which would contradict \ref{item:b.2} being satisfied.
	Then, it has to be that $\lim\limits_{t \rightarrow T} \phi(t,J)$ is infinity.
	When \ref{item:star1} holds, $\lim\limits_{t \rightarrow T} \phi(t,J)$ being infinity is a contradiction since $K \cap C$ is compact.
	If \ref{item:star2} holds, there exists $M > 0$ such that $\sup \{\eta: |\eta| \in F(x), x \in K \cap C\} \leq M$.
	Thus, every solution to $\dot{x} \in F(x), x \in K \cap C$ does not exhibit a finite escape time.
	If \ref{item:star3} holds,  \cite[Lemma 1]{aubin.hs.viability},\footnote{The sets $X, K, C$ in \cite[Lemma 1]{aubin.hs.viability} are $C, K \cap C, \overline{K \cap C \cap D}$, respectively, in our context.} see also \cite[Theorem 3.3.5]{aubin.viability}, implies that $t \mapsto \phi(t,J)$ is either:
	\begin{itemize}[leftmargin = 4mm]
		\item defined over $[t_J, \infty)$ with values in $K\cap C$; or
		\item defined over $[t_J, T]$ with $\phi(T, J) \in \overline{K \cap C \cap D}$ and $\phi(T, J) \in K\cap C$ for every $t \in [t_J,T]$.
	\end{itemize}
	In either case, we have a contradiction.
\end{proof}
}

%\begin{remark}\label{rem:marchaud}
	Note that condition \ref{item:star3} is typically assumed in the study of viability and invariance of differential inclusions; see, e.g., \cite{aubin.viability, aubin.hs.viability, aubin2009set}.
	Condition \ref{item:star1} and \ref{item:star2} do not require $F$ to be Marchaud, but impose boundedness of $F$ and extra properties on $K \cap C$.
	In fact, besides \ref{item:star3} providing an alternative condition for \ref{item:N*}, linear growth is not imposed on $F$ in this paper.
%	In Lemma~\ref{lem:star}, we require $F$ to be outer semicontinuous, locally bounded, and with nonempty, convex image, which imply that $F$ enjoys all properties of being Marchaud except for the linear growth.
%\end{remark}

The next example illustrates Theorem~\ref{thm:wfi} and Lemma~\ref{lem:star}.
\begin{example}(weakly forward invariant set)\label{ex:wFI}
	Consider the hybrid system $\HS = \data$ in $\reals^2$ given by
	\begin{align*}
		&F(x):= (x_2, -x_1) & \forall x \in C;\\
		&G(x):= (-0.9x_1, x_2) &\forall x \in D,
	\end{align*}
	where $C := \{x \in \reals^2: |x| \leq 1, x_2 \geq 0\}$ and
	$D:= \{x \in \reals^2: x_1 \geq -1, x_2 = 0\}.$
	\vspace{-7mm}
	\begin{figure}[H]
		\centering
		%			\setlength{\unitlength}{.3\textwidth}
		\includegraphics[width=\figsize]{wFI.eps}
		\small
		\put(-0.05,.12){$x_1$}
		\put(-.62,.5){$x_2$}
		\put(-.26,.05){1}
		\put(-.93,.05){-1}
		\put(-.6,.05){0}
		\put(-.7,.3){$C$}
		\put(-.45,.03){$D$}
		\caption{Sets and directions of flows/jumps in Example~\ref{ex:wFI}.}
		\label{fig:wFI}
	\end{figure}
	\vspace{-3mm}

	\noindent The set $K = \partial C$ is weakly forward invariant for $\HS$ by Theorem~\ref{thm:wfi}.
	More precisely, for every $x \in K \cap D$, $G(x) \subset K$; and for every $x \in K \setminus D = \{x \in \reals^2:  |x| = 1, x_2 > 0\}$, since $\inner{\nabla( x^2_1 + x^2_2)}{F(x)} = 0$, $F(x) \subset T_{K \cap C}(x)$.
	In addition, $K \cap C = \partial C$ is compact, which implies condition \ref{item:N*} holds by Lemma~\ref{lem:star}.
	Thus, for every $x \in K$, there exists one maximal solution that is complete and stays within $K$.
	One such maximal solution starts from $(0,1)$ and flows along $|x| = 1$, becomes eventually discrete after reaching $(1,0)$, while staying within $K$.
	In fact, for every point in $\{x\in \reals^2: x_1 \in (-1, 1), x_2 = 0 \}$, there exists one maximal solution that is complete, discrete and stays in $K$ (from the origin there is also a complete continuous solution that remains at the origin), but also there exist maximal solutions that flow inside $\{x \in \reals^2: |x| < 1 \}$ and leave $K$.
	\hfill $\triangle$
\end{example}

Note that because the set $K \cap C$ is closed and that for every $x \in \inter (K \cap C)$, $T_{K \cap C}(x) = \reals^n$, condition
	\begin{enumerate}[label = \ref{thm:fi}.2$^{'}$), leftmargin= 12mm]
		\item\label{item:fi2'} For every $x \in \partial (K \cap C), F(x) \subset T_{K \cap C}(x)$
	\end{enumerate}
implies condition \ref{item:fi2} in Theorem~\ref{thm:fi}.
In addition, one can replace condition \ref{item:fi2} in Theorem~\ref{thm:fi} by
	\begin{enumerate}[label = \ref{thm:fi}.2$^{''}$), leftmargin= 12mm]
		\item\label{item:fi2''} For every $x \in \partial (K \cap C),$
	\end{enumerate}
	\vspace{-6mm}
	\begin{align}
		& F(x) \subset T_{K \cap C}(x) &\ifeq &x \notin \partial C \cap D\label{eq:fi2''}\\
		&F(x) \cap (T_C(x) \setminus T_{K \cap C}(x)) = \emptyset  &\ifeq &x \in \partial C \cap D. \label{eq:fi2''s}
	\end{align}
This replacement allows us to verify forward invariance of $K = C$ for the hybrid system $\HS$ in Example~\ref{ex:wFI}:
even though $F(x) \cap T_{K \cap C}(x) = \emptyset$ at every $x \in \{x \in \reals^2:  x_2 = 0, 0 < x_1 \leq 1 \}$, the solutions can be extended by jumping when reaching the positive $x_1-$axis.
Note that assumption \eqref{eq:fi2''s} is important as in some cases, having item \eqref{eq:fi2''} only leads to solutions that escape the set $K$ by flowing as shown in the following example.
Consider the hybrid system $\HS$ on $\reals^2$ with
\IfConf{
	system data given by
	$F(x) =(x_2, -\gamma)$, $C := \{x \in \reals^2: x_1x_2 \geq 0 \}$,
	$G(x) = x$ and $D := \{x \in \reals^2: x_1 \geq 0, x_2 = 0 \},$
	}{
\begin{align*}
	&F(x) =(x_2, -\gamma) & \forall x &\in C := \{x \in \reals^2: x_1x_2 \geq 0 \}\\
	&G(x) = x & \forall x &\in D := \{x \in \reals^2: x_1 \geq 0, x_2 = 0 \},
\end{align*}
}
where $\gamma > 0$.
The set $K = \{x \in \reals^2: x_1 \geq 0, x_2 \geq 0 \}$ is weakly forward invariant, and the sets $K, C, D$ and the map $F$ satisfy condition \ref{item:fi2''}.
However, at the origin, we have $F(0) = (0, -\gamma)$ and
\vspace{-1mm}
\begin{align*}
	&T_C(0) = (\reals_{\geq 0} \times \reals_{\geq 0} ) \cup (\reals_{\leq 0} \times \reals_{\leq 0}),\\
	&T_{K \cap C}(0) = \reals_{\geq 0} \times \reals_{\geq 0}.
\end{align*}
\vspace{-5mm}

\noindent Hence, at the origin, one solution can flow into $C \setminus K$ (the third quadrant) because $F(0) \in T_C(0) \setminus T_{K \cap C}(0)$.
%In addition, for some cases, it might be possible to further relax \ref{item:fi2'} to
%\begin{enumerate}[label = \ref{thm:fi}.2''), leftmargin=3.2\parindent]
%	\item\label{item:fi2''} For every $x \in (\partial (K \cap C)) \setminus (\partial C \cap D)$, $ F(x) \subset T_{K \cap C}(x)$.
%\end{enumerate}
%For example, the hybrid system $\HS$ given in Example~\ref{ex:wFI} is such that \ref{item:fi2''} holds for $K = C$ and the set $K$ is forward invariant.
%This is because even though $F(x) \cap T_{K \cap C}(x) = \emptyset$ at every $x \in \{x \in \reals^2:  x_2 = 0, 0 < x_1 < 1 \} \subset K \cap \partial C$, the solutions can be extended by jump when reaching the positive $x_1-$axis.
%On the other hand, replacing \ref{item:fi2} by \ref{item:fi2''} in general is not obvious.
%In fact, in some cases, a solution may flow out of the set $K$ from a point $x \in K \cap \partial C$ such that $F(x) \cap T_{K \cap C}(x) = \emptyset$.
%\ricardo{It seems we could prove that when 
%$F(x) \cap (T_C(x) \setminus T_{K \cap C}(x)) = \emptyset$
%then \ref{item:fi2''} implies \ref{item:fi2}, no? In that case,
%we could show forward invariance of
%the set $K = [0,1]$ for
%$\HS$ with data $C = K$, $f(x) = 1$, $D = \{1\}$, and $G(x) = 0$
%which our conditions in Theorem~\ref{thm:fi} do not allow to show.
%}
%This is due to the fact that, for example, when $C$ is closed, we may have $F(x) \cap (T_C(x) \setminus T_{K \cap C}(x)) \neq \emptyset$ 
%\ricardo{in $K \cap \partial C$, right?:}at such $x$.
%To illustrate this point, consider the hybrid system $\HS$ on $\reals^2$ with
%	\begin{align*}
%		&F(x) =(x_2, -\gamma) & \forall x &\in C := \{x \in \reals^2: x_1x_2 \geq 0 \}\\
%		&G(x) = x & \forall x &\in D := \{x \in \reals^2: x_1 \geq 0, x_2 = 0 \},
%	\end{align*}
%	where $\gamma > 0$. The set $K = \{x \in \reals^2: x_1 \geq 0, x_2 \geq 0 \}$ is weakly forward invariant, and the sets $K, C, D$ and the map $F$ satisfy condition \ref{item:fi2''}.
%However, at the origin, we have $F(0) = (0, -\gamma)$ and
%	\begin{align*}
%		&T_C(0) = (\reals_{\geq 0} \times \reals_{\geq 0} ) \cup (\reals_{\leq 0} \times \reals_{\leq 0}),\\
%		&T_{K \cap C}(0) = \reals_{\geq 0} \times \reals_{\geq 0},
%	\end{align*}
%which indicate that a solution can flow into $C \setminus K$ (the third quadrant) because $F(0) \in T_C(0) \setminus T_{K \cap C}(0)$.
%Hence, \ref{item:fi2} does not hold and $K$ is not forward invariant.

The following example is an application of Theorem~\ref{thm:fi} and Lemma~\ref{lem:star}.
\begin{example}(forward invariant set)\label{ex:oscillator0w}
	Consider the hybrid system given by
	\IfConf{
		\begin{align}\label{eq:ex_zerod}
			\HS \begin{cases}
				x \in C &\dot{x} = F(x) := (- |x_1|x_2, 0)\\
				x \in D & x^+ = G(x) := x,
			\end{cases}
		\end{align}
		}{
	\begin{align}\label{eq:ex_zerod}
		\HS \begin{cases}
			x \in C &\dot{x} = F(x) := \begin{bmatrix}- |x_1|x_2 \\ 0
			\end{bmatrix} \\
			x \in D & x^+ = G(x) := x,
		\end{cases}
	\end{align}
}
	where the flow set is $C = \{x \in \reals^2:  |x| \leq 1, x_1x_2 \geq 0 \}$ and the jump set is $D = \{x \in \reals^2:  |x| \leq 1, x_1x_2 \leq 0 \}$.
	We observe that during flow, solutions evolve continuously within the unit circle centered at the origin; while at jumps, solutions remain at the current location.
	Applying Theorem~\ref{thm:fi}, we show that the set $K_a = C_1 \cup D_1$ is forward invariant for $\HS,$ where $C_1 = \{x \in \reals^2: x_1 \geq 0, x_2 \geq 0, |x| \leq 1\}$ and $D_1 = \{x \in \reals^2: x_1 \leq 0, x_2 \geq 0, |x| \leq 1\}$.
	By construction, $K_a, C, D$ and $F$ satisfy Assumption~\ref{assum:data}. 
	Condition \ref{item:fi1} holds since $G$ maps the state to its current value.
	Condition \ref{item:fi2} holds since
	\begin{itemize}[leftmargin = 4mm]
		\item for every $x \in \inter (C_1)$, $T_{K_a \cap C}(x) = \reals^2$;
		\item for every $x \in \{x \in  \partial C_1: |x| =1 \}$, inner product between the gradient of $x^2_1 + x^2_2$ and $F(x)$ is nonpositive, i.e.,
		\begin{align*}
		\inner{\nabla (x_1^2 + x_2^2)}{F(x)} &= -2|x_1|x_1x_2 \leq 0
		\end{align*}
		because $x_1 x_2 \geq 0$, which implies $F(x) \in T_{K_a \cap C}(x);$
		\item for every $x \in \{x \in  \partial C_1: |x| \neq 1 \}$, we have that 
		$$T_{K_a \cap C}(x) = 
		\begin{cases}
		\reals_{\geq 0} \times \reals & \ifeq x_1 = 0, x_2 \notin \{0,1\}\\
		\reals \times \reals_{\geq 0} & \ifeq x_1 \notin \{0,1\}, x_2 = 0\\
		\reals_{\geq 0}^2 & \ifeq x = 0,
		\end{cases}$$
		which implies $F(x) \in T_{K_a \cap C}(x)$ holds.
	\end{itemize}
	Finally, item \ref{item:star1} in Lemma~\ref{lem:star} holds for $K_a$ and $C$, thus, \ref{item:N*} holds.
	%		Then, with similar analysis, we can verify the forward invariance of set $K_2$ for the zero disturbance case of system in Example~\ref{ex:reoscillator}. Namely, the flow set of $\HS$ in \eqref{eq:ex_zerod} is replaced by $C' = \{x \in \reals^2: |x| \leq 1 \}$ Applying Theorem~\ref{thm:fi}, Assumption~\ref{assum:data} and condition \ref{item:N*} hold for $K_2, F, C'$ and $D$. Moreover, the map $F$ is locally Lipschitz on $C'$ by construction. Then, condition \ref{item:fi1} holds since for every $x \in K_2 \cap D$, the map $G$ does not change the value of state $x$. Condition \ref{item:fi2} holds since for every $x \in K_2 \cap C$, the map $F$ is such that 
	%		\begin{itemize}
	%			\item for every $x \in \inter (K_2 \cap C') = \inter C_1$, $T_{K_2 \cap C'} = \reals \times \reals$;
	%			\item for every $x \in \partial (K_2 \cap C')$, the inner product between the circle and the map $F(x)$ is non-positive, i.e., 
	%			\begin{align*}
	%				\inner{\nabla (x_1^2 + x_2^2)}{F(x)} &= 2x_1(-x_2) \leq 0
	%			\end{align*}
	%			because $x_1 x_2 \geq 0$, which implies 
	%			$$\Fw(x) \in T_{K_2 \cap C'}(x).$$ %%%%%% Not true since No constraint $x_1 x_2 \geq 0$
	%		\end{itemize}
	%		Thus, the set $K_2$ is robustly forward invariant for $\HS.$
	\hfill $\triangle$
\end{example}

	In Example~\ref{ex:oscillator0w}, the set $K_a$ is forward invariant for $\HS$ as shown above.
	When arbitrarily small disturbances are introduced, solution pairs may escape the set of interest.
	In particular, we revisit Example~\ref{ex:oscillator0w} with disturbances in the next section, and show that $K_a$ is only weakly forward invariant uniformly in the given disturbances.
	The forthcoming results in Section~\ref{sec:HwSuffConds} are useful to verify such properties of sets for hybrid systems $\Hw$ given as in \eqref{eq:Hw}.
%%%%%%%%%%%%%%%%%%% Nominal case proofs %%%%%%%%%%%%%%
%%\NotConf{This result follows from an application of Theorem~\ref{thm:rwFI} for a hybrid system with zero disturbance. An proof that is independent of Theorem~\ref{thm:rwFI} for Theorem~\ref{thm:wfi} is provided as follows.
%%	\begin{proof}
%%		Given $K, C, D, F$  satisfying Assumption~\ref{assum:data}, we define the restriction of $\HS$ by $K$, i.e., $\widetilde{\HS} = (\widetilde{C} , F , \widetilde{D}, G)$, where $\widetilde{C} := K\cap C$ and $\widetilde{D} := K\cap D$. Let $K_1 = \widetilde{D} $ and $K_2 = K\setminus D$. By an application of \cite[Lemma 5.26]{hybridbook}, conditions in Assumption~\ref{assum:data}, i.e., $K \cap C$ is closed, $F$ is outer semicontinuous, locally bounded relative to $K \cap C$, and $F(x)$ is convex for every $x \in K \cap C$, and item \ref{item:wfi2} together imply that \ref{item:(VC} in Proposition~\ref{prop:existence} holds for every $x \in K_2$. Then, since $K = K_1 \cup K_2$ and $K \subset \overline{C}\cup D$, applying Proposition~\ref{prop:existence}, there exists a nontrivial solution $\phi$ from every point of $K$. In addition, for every $\xi \in K$, we construct a nontrivial $\widetilde{\phi} \in {\cal S}_{\widetilde{\HS}}(\xi)$ such that $\rge  \widetilde{\phi} \subset K$. Since $K_1 \cap K_2 = \emptyset$, we have the following two cases:
%%		\begin{enumerate}[i)]
%%			\item If $\xi \in K_1$, then $\xi \in D$; hence, a jump is possible from every $\xi$ in $K_1$. Let $\widetilde{\phi}(0,0) = \xi$. By condition \ref{item:wfi1}, there exists $\widetilde{\phi}(0,1) \in G(\xi)$  such that $\widetilde{\phi}(0,1) \in K$.
%%			\item If $\xi \in K_2$, then $\xi \in \overline{C}\setminus D$ and nontrivial solutions can only evolve by flowing. Since (VC) holds for every $\xi \in K_2$, there exist $\varepsilon > 0$ and $z: [0,\varepsilon] \rightarrow \reals^n$ with the properties in \ref{item:(VC}. Then, $\widetilde{\phi}$ with $\widetilde{\phi}(0,0) = \xi$ and $\widetilde{\phi}(t,0) = z(t)$ for all $t \in [0, \varepsilon]$ is a nontrivial solution to $\widetilde{\HS}$.
%%		\end{enumerate}
%%		The above shows that there exists a nontrivial solution from every point in $K$. It also shows that from every point in $K_1$, solutions can be extended to continue jumping in $K_1$ using the construction in case i), while from points in $K_2$, solutions can be extended using the construction in case ii). Moreover, since $K \cap C$ is closed, by definition of solutions, such extensions can be defined so as they do not leave $K_2$ by flowing (since they can always be extended using the argument in ii)). As a consequence, from every $\xi \in K$, there exists at least one maximal solution $ \widetilde{\phi}$ to $\widetilde{\HS}$ that stays in $K$. 	
%%		
%%		Next, we prove that each such $  \widetilde{\phi}$ is also a maximal solution to $\HS$. If $  \widetilde{\phi}$ is complete, then $\widetilde{\phi}$ is already maximal. Consider the case that $  \widetilde{\phi}$ is not complete. Proceeding by contradiction, suppose $\widetilde{\phi}$ is not maximal for $\HS$, meaning that there exists $\phi$ such that $\phi(t,j) =   \widetilde{\phi}(t,j)$ for every $(t,j)\in \dom \widetilde{\phi}$ and $\dom \phi \setminus \dom \widetilde{\phi} \neq \emptyset$. Let $(T,J) = \sup \dom   \widetilde{\phi}$. If $(T,J) \in \dom   \widetilde{\phi}$, since $  \widetilde{\phi}(T,J) \in (C\cup D)\cap K$, conditions \ref{item:wfi1} and \ref{item:wfi2} imply that, using the arguments in i) and ii) above, it is possible for $\phi$ to satisfy $\phi(t,j) \in K$ for $(t,j) \in \dom \phi \setminus \dom   \widetilde{\phi}$, which, by definition of solutions, contradicts the maximality of $  \widetilde{\phi}$ for $\widetilde{\HS}$. If $(T,J) \notin \dom   \widetilde{\phi}$, according to Proposition~\ref{prop:existence}, \ref{item:b.2} holds. In such a case, since $\lim\limits_{t+j \rightarrow T+J} \phi (t,j) \in K \cap C$ and $K \cap C$ is closed, an extension of $  \widetilde{\phi}$ outside of $K$ is not possible, which is a contradiction to the definition of $\phi$. Thus, $K$ is weakly forward pre-invariant for $\HS$.
%%		
%%		Finally, we prove that $K$ is weakly forward invariant for $\HS$ when, in addition, $\HS$ and $K$ satisfy condition \ref{item:N*}. We proceed by showing that from every $\xi \in K$ there exists at least one complete solution $\phi$ for the $K$ restricted system $\widetilde{\HS}$. This is because such complete solutions are also maximal for the original system $\HS$ and have $\rge \phi \subset K$. The existence of nontrivial solutions to $\widetilde{\HS}$ from every $\xi \in K$ is guaranteed by the fact that $K$ is weakly forward pre-invariant for $\HS$. By the closedness of $K \cap C$ and continuity of the function $z$ in \ref{item:(VC} of Proposition~\ref{prop:existence}, for every $\xi \in K \setminus D$ case \ref{item:b.1} is excluded for some $\phi \in {\cal S}_{\widetilde{\HS}}(\xi)$. Moreover, case \ref{item:b.2} does not hold for all maximal solutions as required by condition \ref{item:N*}. Due to condition \ref{item:wfi1}, from every $\xi \in K\cap D$, at least one solution can be extended by jumping to points in $G(x) \cap K$, from where the solution can be extended either by jumping or flowing afterward. Thus, case \ref{item:c} in Proposition~\ref{prop:existence} is not possible for such solutions. Hence, according to Proposition~\ref{prop:existence}, for each $\xi \in K$, there exists $\phi \in {\cal S}_{\widetilde{\HS}}(\xi)$ such that only \ref{item:a} holds.
%%	\end{proof}
%%}
%
%%\NotConf{This result follows from an application of Theorem~\ref{thm:rFI} for a hybrid system with zero disturbance. An proof that is independent of Theorem~\ref{thm:rFI} for Theorem~\ref{thm:fi} is provided as follows.
%%	\begin{proof}
%%		Since conditions \ref{item:fi1} and \ref{item:fi2} imply conditions \ref{item:wfi1} and \ref{item:wfi2} in Theorem~\ref{thm:wfi}, respectively, under Assumption~\ref{assum:data}, there exist one nontrivial solution to $\HS$ from every point in $K$. Next, proceeding by contradiction, we show that $K$ is forward pre-invariant for $\HS$ when conditions \ref{item:fi1} and \ref{item:fi2}  hold. Suppose there exists a solution $\phi \in {\cal S}_{\HS}(K)$ such that $\rge \phi \setminus K \neq \emptyset$. Then, there exists $(t^*, j^*) \in \dom \phi$ such that $\phi(t^*,j^*) \notin K$, i.e., $\phi$ eventually leaves $K$ in finite hybrid time.
%%		%\footnote{Note that when $\rge \phi \subset K$ and $\lim\limits_{t+j \to \sup_t \dom \phi + \sup_j \dom \phi} \phi(t,j) = \infty$ (that is, $\phi$ stays in $K$ but escapes to infinity, potentially in finite hybrid time) corresponds to a solution that satisfies the definition of forward invariance for $K$.} 
%%		We have the following cases:
%%		\begin{enumerate}[i)]
%%			\item The solution $\phi$ ``leaves $K$ by jumping:'' namely, $\phi(t,j) \in K$ for all $(t,j) \in \dom\phi$ with $t+j < t^* +j^*$, and $\phi(t^*,j^*-1) \in K\cap D$. Since $\phi(t^*,j^*-1) \in K \cap D$, item \ref{item:fi1} implies $\phi(t^*,j^*) \in K$, which is a contradiction.
%%			% Then, it must be the case that $\phi$ left $K$ by flowing. We consider this possibility in the next item.
%%			\item The solution $\phi$ ``leaves $K$ by flowing:'' by definition of solution, $\phi$ leaves $K\cap C$ and enters $\overline{C}\setminus K$. Then, there exists a hybrid time instant $(\tau^*,j^*) \in \dom \phi$ such that $\phi(t,j^*) \in \overline{C}\setminus K$ for all $t \in (\tau^*,t^*]$ and $\tau^* < t^*$ is arbitrarily small and positive. Moreover, by closedness of $K\cap C$, $\phi(\tau^*,j^*) \in \partial (K \cap C)$.
%%			Let $t \mapsto \chi(t) \in K \cap C$ be such that for every $t \in [\tau^*, t^*]$,
%%			\begin{align}\label{eq:chi*}
%%			|z(t)|_{K\cap C} = |z(t)-\chi(t)|,
%%			\end{align}
%%			where $z(t) = \phi(t,j^*)$ for all $t \in [\tau^*, t^*]$. The function $\chi$ exists because of the closeness of $K \cap C$. Since $\phi$ is a solution to $\HS$, the function $t \mapsto |z(t)|_{K\cap C}$ is absolutely continuous. Thus, for almost every $t \in  [\tau^*, t^*]$, $\frac{d}{dt}|z(t)|_{K\cap C}$ exists. Let $t$ be such that both $\frac{d}{dt}|z(t)|_{K\cap C}$ and $\dot{z}(t)$ exist. Because $\dot{z}(t) \in F(z(t))$, we have that the Dini's derivative of $|z(t)|_{K \cap C}$ is
%%			\begin{align*}
%%			\frac{d}{dt}|z(t)|_{K\cap C} &= \lim\limits_{ t' \searrow t} \frac{|z(t')|_{K\cap C} - |z(t)|_{K\cap C} }{t'-t}\\
%%			&= \liminf\limits_{h \searrow 0} \frac{|z(t+h\dot{z}(t))|_{K\cap C} - |z(t)|_{K\cap C} }{h},
%%			\end{align*}
%%			which, by the properties of $\chi$ in \eqref{eq:chi*}, satisfies 
%%			\begin{align*}
%%			&\!\!\!\!\!\!\!\!\! \frac{|z(t) + h\dot{z}(t)|_{K\cap C} - |z(t)|_{K\cap C}}{h} \\
%%			& \leq \frac{|z(t) - \chi(t)| + |\chi(t)+h\dot{z}(t)|_{K\cap C} - |z(t)|_{K\cap C}}{h} =  \frac{|\chi(t)+h\dot{z}(t)|_{K\cap C}}{h}\\
%%			&\leq \frac{|\chi(t)+h\omega|_{K\cap C}}{h} + |\dot{z}(t) - \omega|,
%%			\end{align*}
%%			for every $\omega \in T_{K\cap C}(\chi(t)).$ By definition of the tangent cone in \eqref{eq:tangent}, we have
%%			\begin{align*}
%%			\frac{d}{dt}|z(t)|_{K\cap C} 
%%			\leq \liminf\limits_{h \searrow 0} \frac{|\chi(t)+h\omega|_{K\cap C}}{h} + |\dot{z}(t) - \omega| 
%%			= |\dot{z}(t) - \omega|, 
%%			\end{align*}
%%			for every $\omega \in T_{K\cap C}(\chi(t))$. Thus, for almost every $t \in  [\tau^*, t^*]$,
%%			$$\frac{d}{dt}|z(t)|_{K\cap C} \leq |\dot{z}(t)|_{T_{K\cap C}(\chi(t))}.$$
%%			Since $K \cap C$ is closed, by definition, $\chi(t) \in K \cap C$ for every $t \in [\tau^*, t^*]$. Condition \ref{item:fi2} implies that for almost all $t \in  [\tau^*, t^*]$, we have
%%			\begin{align*}
%%			\frac{d}{dt}|z(t)|_{K\cap C} 
%%			&\leq |\dot{z}(t)|_{T_{K\cap C}(\chi(t))} \leq |\dot{z}(t)|_{F(\chi(t))}.
%%			\end{align*}
%%			Since $t^* - \tau^*$ is positive and can be arbitrarily small, it is always possible to construct a neighborhood of $\chi(t)$ for every $t \in [\tau^*, t^*]$, denoted $U$, with $z(t) \in U$, and there exists a constant $\lambda > 0$ satisfying
%%			$$F(z(t)) \subset F(\chi(t)) + \lambda|z(t)- \chi(t)|\ball,$$
%%			for every $t \in [\tau^*, t^*]$. Hence, for every $t \in [\tau^*, t^*]$, and every $\eta \in F(z(t))$,
%%			$$|\eta|_{F(\chi(t))} \leq \lambda|z(t)- \chi(t)|.$$
%%			Moreover, since $\dot{z}(t) \in F(z(t))$, we have that 
%%			$$|\dot{z}(t)|_{F(\chi(t))} 
%%			\leq \lambda|z(t) - \chi(t)| = \lambda|z(t)|_{F(\chi(t))} .$$
%%			Then, by the Gronwall Lemma (see, e.g., \cite[Lemma A.1]{khalil.nonlinear.sys}), for every $t \in  [\tau^*, t^*]$,  
%%			$$|z(t)|_{K \cap C} = 0.$$ 
%%			Since $K \cap C$ is closed, $\phi(t^*,j^*) \in K \cap C$, which contradicts the definition of $t^*$. Thus, for every $x \in K \cap C$, there does not exist a maximal solution $\phi \in \sol_{\HS}(K)$ that eventually leaves $K\cap C$ by flowing.
%%		\end{enumerate}
%%		Therefore, every $\phi \in {\cal S}_{\HS}(K)$ is such that $\rge \subset K$.
%%		
%%		To complete the proof, we show that when $\HS$ and $K$ also satisfy condition \ref{item:N*}, the set $K$ is forward invariant for $\HS$. Since there exists a nontrivial solution from every point in $K$, we show that only case \ref{item:a} in Proposition~\ref{prop:existence} holds for every $\phi \in {\cal S}_{\HS}(K)$. Proceeding by contradiction, suppose that there exists $\phi^* \in {\cal S}_{\HS}(K)$ that is not complete. Let $(T,J) = \sup \dom \phi^*$ and $T+ J < \infty$. By the closedness of $K \cap C$, $\phi^*$ does not end as described in case \ref{item:b.1}. Since $K$ is forward pre-invariant for $\HS$, every $\phi \in {\cal S}_{\HS}(K\cap C)$ is such that $\rge \subset K$. Using arguments similar to those in the proof of Theorem~\ref{thm:wfi}, case \ref{item:b.2} does not hold for $\phi^*$ by virtue of condition \ref{item:N*}. Then, according to Proposition~\ref{prop:existence}, $\phi^*$ satisfies \ref{item:c} therein. But \ref{item:fi1} leads to a contradiction of the maximality of $\phi^*$. More precisely, item \ref{item:fi1} implies that $G(\phi^*(T,J-1)) \subset K$, so $\phi^*(T,J) \in K \subset \overline{C}\cup D$, and, hence, the solution $\phi^*$ can be extended either by flow or jump using the arguments in i) and ii) of proof for Theorem~\ref{thm:wfi}. Thus, by an application of Proposition~\ref{prop:existence}, all maximal solutions to $\HS$ that start from $K$ are complete and have $\rge \phi \subset K$.
%%	\end{proof}
%%}
